Analysing properties of the C. Elegans neural network: mathematically modeling a biological system

The brain is one of the most studied and highly complex systems in the biological world. It is the information center behind all vertebrate and most invertebrate life, and thus has become a major focus in current research. While many of these studies have concentrated on studying the brain directly, our focus is the structure of the brain itself: at its core an interconnected network of nodes (neurons). A better understanding of the structural aspects of the brain should elucidate some of its functional properties. In this paper we analyze the brain of the nematode Caenorhabditis elegans. Consisting of only 302 neurons, it is one of the better-understood neural networks. Using a Laplacian matrix of the 279-neuron "giant component" of the network, we use an eigenvalue counting function to look for fractal-like self similarity. This matrix representation is also used to plot (in eigenfunction coordinates) both 2 and 3 dimensional visualizations of the neural network. Further analysis examines the small-world properties of the system, including average path length and clustering coefficient. We then test for localization of eigenfunctions, using graph energy and spacial variance. To better understand these results, all of these calculations are also performed on random networks, branching trees, and known fractals, as well as fractals which have been "rewired" to have small-world properties. This analysis is one of many stepping-stones in the research of neural networks. While many of the structures and functions within the brain are known, understanding how the two interact is also important. A firmer grasp on the structural properties of the neural network is a key step in this process

==> Methods.tex <==
\section{Methods}\label{methods}
In order to analyze only the framework of the \emph{C. elegans} neural network, we constructed a Laplacian matrix derived form the adjacency matrices in [30].  We wanted to look only at linkage between neurons, regardless of connection type or direction.  The network of chemical synapses sends signals in one direction only, resulting in a non-symmetric adjacency matrix, $C$.  In order to disregard this directionality, we added this matrix to its own transpose, $C'$, creating a symmetric matrix indexing all chemical connections.  We added this matrix to the adjacency matrix of the gap junction system, $G$ (which is already symmetric because these connections are bidirectional).  

\[
B=[b_{i,j}]= (C+CÕ)+G  \text{ such that } i,j\leq279
\]

We then normalized all non-zero entries of this combined matrix, $B$, to be 1 (in order to un-weight connections), resulting in an adjacency matrix representing the framework of the entire network, $A$.  

\[
A=[a_{i,j}]  \text{ where }  a_{i,j}=b_{i,j}/b_{i,j} if b_{i,j}>0, \text{ otherwise }  a-{i,j}=0 /text{ when } b_{i,j}=0
\]

It is then simple to produce a laplacian matrix, $L$, as shown below:

\[
d_{j}=\sum_{i=1}^{i=279} a_{i,j} \text{ for each } j\leq279
\]Note that $d_{j}$ is the degree of each vertex {j}.  The degree matrix, $D$, is now defined as:

\[
D=[d_{i,j}] \text{ where } d_{i,j}=d_{j} \text{ when } i=j \text{ and } d_{i,j}=0 \text{ when } i\neqj
\]

Then the laplaican matrix, $L$, is given by:

\[
L=D-A
\]

\subsection{The Eigenvalue Counting Function and Weyl Ratios}

	For a given graph laplacian matrix, $L$, the eigenvalue counting function, $N(x)$ is a cumulative frequency function on the spectrum of the matrix where:
\[
N(x) = \#\{\lambda_{j} \leq x\} \text{ where each } \lambda_{j}  \text{ is an eigenvalue of } L
\]
The growth of $N(x)$ is approximately $x^\alpha$, thus the relevant portion of each graph, when using a logarithmic scale, appears to be linear.  A line of best fit was found for each relevant interval, and the slope, $\alpha$, calculated.  Using this $\alpha$, we plotted the Weyl ratio, $W(x)$, such that:
\[
W(x)= N(x)/x^{\alpha}.
\]
These Weyl ratios allow us to examine the spectrum of each matrix, looking for elements such as symmetry and periodicity. [26]

\subsection{Normalizing a Laplacian Matrix}

	We used two different forms of these matrices: both the standard Laplacian matrix and the degree-normalized Laplacian.  In the case of eigen projections, we utilize the degree-normalized matrix.  We define the degree matrix, $D$, as before: a diagonal matrix whose non-diagonal elements are 0, and each entry $d_{j,j}$ is the degree of the $j^{th}$ vertex. Using both the standard Laplacian, $L$ and its corresponding degree matrix, $D$, we produce the degree-normalized Laplacian, $Q$:
\[
Q = D^{(-1/2)} L D^{(-1/2)}
\]
Using the degree-normalized Laplacian has mainly aesthetic advantages, as shown in Figure 678

\subsection{Graphing in Eigenfunction Coordinates}

	We found all eigenvalues, $\lambda_k$, and their corresponding eigenfunctions, $\varphi_k$, for each matrix.  Given two eigenfunction $\varphi_i$ and $\varphi_j$, we then plotted the ordered pair $(\varphi_i(n), \varphi_j(n))$ for each $n$ from 1 to 279, as described in [Begue].  The first eigenvalue of any Laplacian matrix is always 0, corresponding to a constant eigenfunction.  Thus we only consider $\varphi_i$ and $\varphi_j$ with $i ,j \geq 2$.  Edges were then added between points to represent relevant connections, and the same color-coding as [25] was used: where red represents sensory neurons, green are motor neurons, and blue indicates interneurons.  The same process was then repeated in three dimensions, plotting $(\varphi_i(n), \varphi_j(n), \varphi_k(n))$ for some $i, j, k \geq 2$, such that $i\neqj\neqk$.

\subsection{Clustering Coefficient}
	The clustering coefficient is a common measure for vertices on a graph. It is typically measured on graphs with unweighted edges.  For a graph $G$ and a given vertex $v$, let $e_v$ denote the number of connections that exist between the neighbors of $v$.  Take $d_v$ as the number of neighbors of $v$ (the degree of vertex $v$). Then the clustering coefficient of vertex $v$, $c_v$, is given by:
\[
c_v =\frac{2e_v}{(d_v (d_v -1))}
\]
Note that total number of possible connections among neighbors of $v $ is $\frac{1}{2 d_v(d_v - 1)}.  

	Therefore the clustering coefficient is essentially the probability that two neighbors of $v$ are connected. For a graph $G$ with $n$ vertices, the average clustering coefficient, $c$, is defined as:
\[
c=\frac{1}{n}\sum_{v=1}^{n} c_v
\]

\subsection{Generating a Related Random Graph for Small-World Analysis} 

	In order to analyze our networks for small world properties, it was useful to compare these graphs to those of similar networks with randomly assigned edges.  Small-world networks are almost as well-connected as random graphs, but possess a surprisingly well-localized structure.  We developed the following algorithm for this process:
		
		For a graph $G$ with $n$ vertices, let $k$= the number of edges on $G$.  Therefore the average number of edges per vertex is $k/n$.  Furthermore, the probability that any two random vertices are connected, $p$, is given by the number of existing connections divided by the total possible connections: 
\[		
p= \frac{k}{(n(n-1))}
\]
Next we generate a random graph, $Rand(G)$, with $n$ vertices and a $p$ probability of connection between two vertices (See [Supplement]).   We then compute $c$ and $l$ for $G$ and $Rand(G)$.
 
$G$ has small-world network properties [33] if: 
 
 1. $l (G)$ > $l (Rand(G))$
 
 and
 
 2. $c (G)$ > > $c (Rand(G))$ where $c (Rand(G)) \approx p$ 

\subsection{The Neighborhood of a Graph}

	On a graph $G$ with $n$ vertices, the neighborhood, $N(m)$ where $m$ is a positive integer, is useful in analyzing small-world networks. A neighborhood of size $m$ around  vertex $v$ is the set of all vertices that can be reached from $v$ in $m$ steps. We shall refer to the number of vertices reachable in $m$ steps as $N_{v}(m)$. To get a sense of the global neighborhood size on the graph, we can average $N_{v}(m)$ over each vertex $v$ in $G$.  This gives us a global $N(m$ for a given $m$:
\[	
N(m)= \frac{1}{n}\sum_{v=1}{n} N_{v}(m)
\]
 It is clear that $N(m)$ is non-decreasing and as long as $G$ is complete, $N(m)$ achieves its maximum, $n$, for finite $m$.

\subsection{Graph Rewiring}

	The rewiring principle can be rigorously explained as follows. We first number each vertex in $G$ from 1 to |G| (where $n=|G|$, $n$ being the total number of vertices). If there is a connection between vertices $u$ and $v$ in $G$, we generate a random number between 0 and 1. If this random number is less than a given probability $p$, then the connection will be rewired.  Without loss of generality assume $u < v$.  We then fix the connection to vertex $u$, and move the connection to another vertex, $k$, such that $u$ and $k$ were not previously connected.

\subsection{Spacial Variance}

	For a graph $G=(V,E$) where $V$ is the set of vertices and $E$ is the set of edges, one can define an arbitrary scalar function $u: V \rightarrow R$. Consequently, one can then define the energy of $u$ associated with the graph.  The energy of $u$ associated with $G$, $\epsilon(u)$  is defined as:
\[
\epsilon(u) =\sum_{x,y \in E)} (u(x)-u(y))^2. 
\]
The energies form a useful tool in comparing the structures of different graphs.

\subsection{Graph Energy}
	
We must first define the reisistance between two vertices on a grah.  Let $G = (V, E)$ be a graph and $x, y \in V$ . Then the resistance between $x$ and $y$, $d(x, y)$, is given by:
\[
d(x, y) = \epsilon(h(x,y))^{-1}
\]
Where $h(x,y)$ is a harmonic function defined as follows:

Let $G = (V,E)$ be a graph and $x,y \in V$. Then the harmonic function corresponding to $(x, y)$ is a scalar function $h(x,y): V \rightarrow R$ such that: 
	
\[
1. h(x,y)(x) = 0
\]
\[ 
2. h(x,y)(y) = 1
\]
\[
3. \epsilon(h)-1, \text{ where } h \text{ is an arbitrary scalar function on } V , \text{ is maximized at } h(x,y).
\]

Using these we can now define the spacial variance of a graph. Again, let $G = (V,E)$ be a graph with $n$ vertices and $u$ be a scalar function on $V$. Let $\gamma$ be a constant. Then the $\gamma^{th}$ spacial variance of $u$ over $G$ is given by:
\[
Var\gamma(u)= \frac{1}{n}\sum_{x,y \in E)} d(x,y) (u(x)-u(y))^2
\]

